A Simple Deterministic Distributed Low-Diameter Clustering

We give a simple, local process for nodes in an undirected graph to form non-adjacent clusters that (1) have at most a polylogarithmic diameter and (2) contain at least half of all vertices. Efficient deterministic distributed clustering algorithms for computing strong-diameter network decompositions and other key tools follow immediately. Overall, our process is a direct and drastically simplified way for computing these fundamental objects.

==> old.tex <==
\section{The Algorithm}

Our algorithm is based on the following idea. Instead of talking about clusters, we will just talk about their centers that we call terminals. At the beginning, every node is a terminal. 

Then in each of the following $b = O(\log n)$ phases we delete at most $n/(2b)$ nodes of $G$ such that in the new graph, terminals with their $i$-th bit equal to $0$ cannot be in the same connected component with terminals with their $i$-th bit equal to $1$. This means that after $b$ phases every terminal is in a separate connected component and this component is the final cluster. 

To make this approach work, we need to control how close the nodes of $G$ are to terminals. This is controlled by the following well-known definition of a ruling set. 


\begin{definition}[Ruling set]
We say that a subset $Q \subseteq V(G)$ is $R$-ruling if every node $v \in V(G)$ satisfies $d(Q, v) \le R$. 
\end{definition}

Our main result is the following lemma that says that we can carry out our plan of deleting $n/(2b)$ nodes of the input graph so as to separate terminals of different $i$-th bit. Moreover, if the set of terminals was $R$-ruling, it is only $R + O(\log^2 n)$ ruling afterwards. 

\begin{lemma}
\label{lemma:main}
Assume that each node of the input graph is equipped with a unique $b$-bit identifier for some $b = O(\log n)$.
Suppose we are given a set of red and blue \emph{terminals} $Q = Q^\fR \sqcup Q^\fB \subseteq V(G)$ such that $Q^\fR \sqcup Q^\fB$ is $R$-ruling for some $R = O(b^3)$. 
Then, there is a deterministic \congest algorithm running in $O(\log^5(n))$ rounds and which outputs some subset $Q'^\fB \subseteq  Q^{\fB}$ of the blue terminals and a set $V' \subseteq V(G)$ which satisfies $Q^\fR \cup Q'^\fB \subseteq V'$ such that the following three properties are satisfied:
\begin{enumerate}
    \item Ruling Property: $Q^\fR \cup Q'^\fB$ is
    $(R+4b^2)$-ruling in $G[V']$.
    \item Separation Property: Each connected component in $G[V']$ contains either no node from $Q^{\fR}$ or no node from $Q'^\fB$.
    \item Deletion Property: It holds that $|V(G) \setminus V'| \le n/(2b)$.
\end{enumerate}
\end{lemma}

Before we prove \cref{lemma:main}, we first show that we can apply the algorithm of \cref{lemma:main} $O(\log n)$ times to compute a clustering which clusters at least half of the vertices into non-adjacent clusters of diameter $O(\log^3 n)$, thus proving MAIN CLUSTERING RESULT.


\begin{proof}[Proof of MAIN CLUSTERING RESULT]
    The algorithm computes two sequences $V_0 := V(G) \supseteq V_1 \supseteq V_2 \supseteq \ldots \supseteq V_b$ and $Q_0 := V(G) \supseteq Q_1 \supseteq \ldots \supseteq Q_b$.
    In general, $Q_i$ is $(i4b^2)$-ruling in $G[V_i]$ for $i \in \{0,1,\ldots,b\}$. In the end, each connected component of $G[V_b]$ will form one cluster of the output clustering. Moreover, each such connected component will contain exactly one node in $Q_b$. As $Q_b$ is $4b^3$-ruling in $G[V_b]$, this implies that each cluster has diameter $O(\log^3 n)$.
    
    
    For $i \in \{0,1,\ldots,b-1\}$, given $(V_i,Q_i)$, we compute $(V_{i+1},Q_{i+1})$ as follows: first, let $Q_i^\fR$ contain all nodes in $Q_i$ with the $(i+1)$-th bit of the identifier being equal to $0$ and $Q_i^\fB$ contain all nodes in $Q_i$ with the $(i+1)$-th bit of the identifier being equal to $1$. Note that $Q_i = Q_i^\fR \sqcup Q_i^\fB$.
    We invoke \cref{lemma:main} with $Q^\fR_{\Lref{lemma:main}} = Q^\fR_i$, $Q^\fB_{\Lref{lemma:main}} = Q^\fB_i$ and $R_{\Lref{lemma:main}} = i(4b^2)$ on input graph $G_{\Lref{lemma:main}} = G[V_i]$. As an output, we obtain sets $Q'^\fB$ and $V'$. We then define $Q_{i+1} = Q^\fR_i \cup Q'^\fB$ and $V_{i+1} = V'$. The guarantees of \cref{lemma:main} then imply that:
    
    \begin{enumerate}
        \item Ruling Property: $Q_{i+1}$ is $((i+1)4b^2)$-ruling in $G[V_{i+1}]$.
        \item Separation Property: Each connected component in $G[V_{i+1}]$ contains either no node from $Q_{i+1}$ with  the $(i+1)$-th bit of the identifier being $0$ or no node from $Q_{i+1}$ with the $(i+1)$-th bit of the identifier being $1$.
        \item Deletion Property: $|V_{i+1}| \geq |V_i| - \frac{n}{2b}$.
    \end{enumerate}
    
    The deletion property together with the fact that $|V_0| = n$ directly implies that $|V_b| \geq \frac{n}{2}$ and therefore at least half of the nodes are clustered. The separation property directly implies that in the end each connected component of $G[V_b]$ contains at most one node of $Q_b$. We already discussed above why this fact together with the ruling property implies that each cluster has diameter $O(\log^3 n)$.
    To compute the output clustering, we invoke the algorithm of \cref{lemma:main} $b = O(\log n)$ times. Hence, the algorithm runs in $O(\log n) \cdot O(\log^5 n) = O(\log^6 n)$ rounds, as needed.
\end{proof}


\paragraph{Algorithm Description} \todo{How to structure it}
Let $t = 2b^2$. 
The algorithm works in $t$ steps and computes a sequence of rooted forests $F_0, F_1, \ldots, F_t$.
The rooted forest $F_0$ is simply a BFS forest rooted at the set of terminals $Q$. 

Next, consider an arbitrary $i \in \{0,1,\ldots,t-1\}$. We now explain how $F_{i+1}$ is computed given $F_i$. In general, each node contained in $F_{i+1}$ is also contained in $F_i$, i.e., $V(F_{i+1}) \subseteq V(F_i)$, and each root of $F_{i+1}$ is also a root in $F_i$. In particular, each root in $F_i$ is contained in $Q$. We say that a tree in $F_i$ is a red tree if its root is in $Q^\fR$ and otherwise, if its root is in $Q^\fB$, we refer to the tree as a blue tree.
Also, we refer to a node in a red tree as a red node and a node in a blue tree as a blue node.
Each red node in $F_i$ will also be a red node in $F_{i+1}$. Moreover, the path to its root is the same in both $F_i$ and $F_{i+1}$.
Each blue node in $F_i$ can (1)\todo{Is this the correct way how to enumerate stuff} either be a blue node in $F_{i+1}$, in which case the path to its root is the same in both $F_i$ and $F_{i+1}$, (2) be deleted and therefore not be part of any tree in $F_{i+1}$, (3) become a red node in $F_{i+1}$.

Let $V_i^{propose}$ be the set which contains each node $v$ which (1) is a blue node in $F_i$, and (2) $v$ is the only node neighboring a red node (in the graph $G$) in the path from $v$ to its root in $F_i$.
For a node $v \in V_i^{propose}$, let $T_v$ be the subtree rooted at $v$ with respect to $F_i$. Note that it directly follows from the way we defined $V_i^{propose}$ that $v$ is the only node in $T_v$ which is contained in $V_i^{propose}$.

Each node in $V_i^{propose}$ proposes to an arbitrary neighboring red tree in $F_i$. Now, a given red tree $T$ in $F_i$ decides to grow if 

\[\sum_{v \in V^{propose}_i \colon \text{$v$ proposes to $T$}} |V(T_v)| \geq \frac{|V(T)|}{2b}.\]

If $T$ decides to grow, then it accepts all the proposals it received, and otherwise $T$ declines all proposals it received.

We now set 

\[V(F_{i+1}) = V(F_i) \setminus \left( \bigcup_{v \in V^{propose}_i, \text{the proposal of $v$ was declined}} V(T_v) \right).\]
\todo{define Vdeleted here?}

Each node in $V(F_{i+1}) \setminus V^{propose}_i$ has the same parent in $F_{i+1}$ and $F_i$, or is a root in both $F_{i+1}$ and $F_i$.
Each node in $V(F_{i+1}) \cap V^{propose}_i$, i.e., each node whose proposal got accepted by some red tree $T$ in $F_i$, changes its parent to be an arbitrary neighboring node in the tree $T$. 
\todo{Where do you wanna define $V^{deleted}_i$}
Note that if a red tree $T$ decides to grow, then the corresponding tree in $F_{i+1}$ contains at least $\left(1 + \frac{1}{2b}\right)|V(T)|$ vertices. Moreover, if $T$ does not decide to grow, then $T$ is also a tree in $F_{i+1}$ and is not neighboring with any blue tree in $F_{i+1}$. This follows from the fact that each blue node neighboring a red tree either becomes a red node or gets deleted. 

We now have fully specified how the rooted forests $F_0, F_1, \ldots, F_t$ are computed.
In the end, we set $V' = V(F_t)$ and we obtain the output set $Q'^\fB$ by only keeping those nodes in $Q^\fB$ that are the root of a blue tree in $F_t$. Note that $Q^\fR \cup Q'^\fB \subseteq V'$, which is one of the conditions of \cref{lemma:main}.



\todo{Maybe some connective text}



\paragraph{Analysis}
For each $i \in \{0,1,\ldots,t\}$ and $u \in V(F_i)$, we define $d_i(u)$ as the length of the path from $u$ to its root in $F_i$.
\todo{Add intuition to claims?}
\begin{claim}[Ruling Claim]
\label{claim:distance_to_root}
For every $i \in \{0,1,\ldots,t\}$, the following holds:
\begin{enumerate}
    \item If $u$ is in a blue tree in $F_i$, then $d_i(u) = d(Q,u)$.
    \item If $u$ is in a red tree in $F_i$, then $d_i(u) \leq d(Q,u) + 2i$.
\end{enumerate}
\end{claim}
In particular, $Q^\fR \cup Q'^\fB$ is $(R+4b^2)$-ruling in $G[V']$.
\begin{proof}
We prove the statement by induction on $i$. The base case $i = 0$ trivially follows from the fact that $F_0$ is a BFS tree rooted at $Q$.


For the induction step, consider an arbitrary $i \in \{0,1,\ldots,t-1\}$.
We show that the statement holds for $i+1$ given that it holds for $i$.

Consider an arbitrary $u \in V(F_{i+1})$. We have to show that $d_{i+1}(u) = d(Q,u)$ in case $u$ is a blue node in $F_{i+1}$ and $d_{i+1}(u) \leq d(Q,u) + 2(i+1)$ in case $u$ is a red node in $F_{i+1}$. The only case where this does not trivially follow from induction is the case that $u$ is a blue node in $F_i$ and a red node in $F_{i+1}$. 
In that case, there exists a node $v \in V^{propose}_i$ such that $u \in T_v$ and the proposal of $v$ was accepted. In particular, $v$'s parent in $F_{i+1}$ is some neighboring node $w$ which is part of some red tree in $F_i$. As $w$ is $v$'s parent in $F_{i+1}$, we have $d_{i+1}(v) = 1 + d_{i+1}(w)$ and as $w$ is in a red tree in $F_i$, we have $d_{i+1}(w) = d_i(w)$. Moreover, the induction hypothesis gives $d_i(w) \leq d(Q,w) + 2i$ and as $v$ is a neighbor of $w$, it trivially holds that $d(Q,w) \leq d(Q,v) + 1$. Combining the four (in)equalities gives \todo{V: picture?}

\[d_{i+1}(v) = 1 + d_{i+1}(w) = 1 + d_i(w) \leq 1 + d(Q,w) + 2i \leq d(Q,v) + 2(i+1).\]

The path between $u$ and $v$ in $F_i$ is the same as the path between $u$ and $v$ in $F_{i+1}$. Hence, $d_{i+1}(u) - d_{i+1}(v) = d_i(u) - d_i(v)$ and therefore

\[d_{i+1}(u) = d_{i+1}(u) - d_{i+1}(v) + d_{i+1}(v) \leq d_i(u) - d_i(v) + d(Q,v) + 2(i+1) \leq d_i(u) + 2(i+1) = d(Q,u) + 2(i+1),\]\todo{V: I would try to say it is clear instead of this calculation}

where the last equality follows from the induction hypothesis.
This finishes the induction. In particular, $d_t(u) \leq d(Q,u) + 2t \leq R + 4b^2$ for every node $u \in V(F_t) = V'$, where we used that $Q$ is $R$-ruling in $G$. As the set of roots of $F_t$ is equal to $Q^\fR \sqcup Q'^\fB$, it follows that $Q^\fR \cup Q'^\fB$ is $(R+4b^2)$-ruling in $G[V']$.
\end{proof}


\begin{claim}(Separation Claim)
\label{claim:tree_size}
No red node in $F_t$ is neighboring a blue node in $F_t$. In particular, each connected component in $G[V']$ contains either no node from $Q^\fR$ or no node from $Q'^\fB$.
\end{claim}
\begin{proof}
    We observed during the algorithm description that each red tree that decides to grow grows by at least a $(1 + \frac{1}{2b})$-factor in a given step. As
    
    \[\left(1 + \frac{1}{2b}\right)^{t} = \left( \left(1 + \frac{1}{2b}\right)^{2b} \right)^{(t/2b)} > 2^{t/2b} = 2^b \geq n,\]
    
    each tree eventually has to stop growing. However, once a tree decides not to grow, it is not neighboring with any blue node and therefore no red node in $F_t$ is neighboring a blue node in $F_t$.
\end{proof}


\begin{claim}[Deletion Claim]
\label{claim:deletion}
It holds that $|V(G) \setminus V(F_t)| = |V(G) \setminus V'| \leq \frac{n}{2b}$.
\end{claim}
\begin{proof}
A node $u$ got deleted in step $i$, i.e., $u \in V(F_i) \setminus V(F_{i+1})$, because of some tree $T$ in $F_i$ which decided to stop growing, as

\[\sum_{v \in V_i^{propose} \colon \text{$v$ proposes to $T$}} |V(T_v)| < \frac{|V(T)|}{2b}.\]

We blaim this tree $T$ for deleting $u$. Note that $T$ only receives blaim in step $i$ and at most $\frac{V(T)}{2b}$ deleted nodes blaim $T$. During the algorithm description, we observed that $T$ is not neighboring any blue node in $F_{i+1}$ and therefore $T$ is also a tree in $F_t$. Hence, each deleted node can blaim one tree $T$ in $F_t$ for being deleted in such a way that each such tree gets blaimed by at most $\frac{1}{2b}|V(T)|$ nodes, which directly proofs the claim.
\end{proof}

\begin{proof}[Proof of \cref{lemma:main}]

\cref{claim:distance_to_root}, \cref{claim:tree_size}, \cref{claim:deletion} together with the fact that $Q^\fR \cup Q'^\fB \subseteq V'$ imply that $(V',Q'^\fB)$ is a valid output. Moreover, each of the $O(\log^2 n)$ steps can be implemented in $O(\log^3 n)$ \congest rounds. This follows because the diameter of each tree in $F_i$ is $O(\log^3 n)$ according to \cref{claim:distance_to_root}. Hence, $V'$ and $Q'^\fB$ can indeed be computed in $O(\log^5 n)$ \congest \todo{How do I get a space after CONGEST?} rounds.
\end{proof}


